Towards a Scalable and Trustworthy Blockchain: IoT Use Case

Recently, blockchain has gained momentum as a novel technology that gives rise to a plethora of new decentralized applications (e.g., Internet of Things (IoT)). However, its integration with the IoT is still facing several problems (e.g., scalability, flexibility). Provisioning resources to enable a large number of connected IoT devices implies having a scalable and flexible blockchain. To address these issues, we propose a scalable and trustworthy blockchain (STB) architecture that is suitable for the IoT; which uses blockchain sharding and oracles to establish trust among unreliable IoT devices in a fully distributed and trustworthy manner. In particular, we design a Peer-To-Peer oracle network that ensures data reliability, scalability, flexibility, and trustworthiness. Furthermore, we introduce a new lightweight consensus algorithm that scales the blockchain dramatically while ensuring the interoperability among participants of the blockchain. The results show that our proposed STB architecture achieves flexibility, efficiency, and scalability making it a promising solution that is suitable for the IoT context.

==> 4_proposed.tex <==
In order to improve the security and reliability of blockchain-based FL, two mechanisms are proposed: (1) a secure sharding process using subjective logic (SSSL) to improve the reliability of FL devices, and (2) a lightweight sharding consensus (LWSC) to improve the security of FL.
\subsection{Key Notations and Assumptions}
Let $O_i^j$ denotes the subjective opinion or trust of a device $i$ and $j$ is the target to which the opinion applies ($i.e.,$ model updates), where $O= \{b,d,u,a\}$ and $b$, $d$, and $u$ respectively represent the belief, disbelief, and uncertainty of $i$, $b+d+u=1$ and $b$, $d$, and $u \in [0,1]$. The parameter $a$ refers to the base rate, it is used to compute the opinion probability expectation value $E(O)=b+au$. Each shard $S$ trains a FL model, where it holds the vector $O_{i,t}^j$ ($i.e.,$ trust in a FL device) during an epoch $t$ with $a$ uncertainty. In the subjective logic, there can be different opinions ($e.g.,$ $ hyper$ $opinions$, $multinomial$ $opinions$, and $binomial$ $opinions$). In this article, we are interested in uncertain binomial opinion (UBO) over binary events ($i.e.,$ valid or invalid update). This is because, in the FL context, the uncertainty about an update is $u \geq 0$. Let $Beta (X, \alpha,\beta)$ corresponds to a beta probability density function \cite{r13}, where
$
\alpha= r+2a$ and
$\beta=  s+2(1-a) 
$. Let $r$ denotes the number of observations of $X$, and $s$ denotes the number of observations of $\bar{X}$.

We assume that each shard can validate one or several updates. Each shard is composed of multiple FL devices that could be either dishonest or honest. These devices are responsible for validating the updates by reaching a consensus. A blockchain consensus is a fault-tolerant mechanism used to reach an agreement between all the devices. Furthermore, we assume that at the beginning, all the shards have equal rate probability $a$ and opinion $O_{i,t}^j$, respectively. In this article, to obtain accurate reputation values of devices, every shard combines its intra-trust opinion with inter-trust option to generate the composite trust value for devices.   
\subsection{Secure Sharding Using Subjective Logic}
Subjective Logic (SL) is one of the prominent probabilistic logic that evaluates trustworthiness of different entities ($i.e.,$ miners/ Fl devices). The SL uses opinions about probability values to determine a subjective belief through belief, disbelief, and uncertainty statements. 
During a time epoch $te$ different from $t$ ($t$ is a fixed value by the model publisher whereas $te$ is a fixed value by the shard devices), the reputation of a FL devices $i$ regarding an update $t$ in a time slot can be expressed as follows: 
\begin {equation}
O_{i \to t}^{te}= \{b_{i \to t}^{te},d_{i \to t}^{te}, u_{i \to t}^{te}\}
\end{equation} 
Based on SL and UBO, we can obtain:

\begin{equation}
\begin{cases}
b_{i \to t}^{te}= \frac{\alpha_i^{te}}{\alpha_i^{te}+\beta_i^{te}} \\
d_{i \to t}^{te}= \frac{\beta_i^{te}+2a-2}{\alpha_i^{te}+\beta_i^{te}} \\ 
u_{i \to t}^{te}= \frac{2}{\alpha_i^{te}+\beta_i^{te}} \\
a= \text{base rate of X}
\end{cases}
\end{equation} 
Note that a dogmatic opinion of the reliability of a device with $u=0$ is equivalent to a defined probability density function ($i.e.,$ trustworthy or untrustworthy). The shard treats a FL device as reliable after $r$ observations of $X$ and $s$ observations of $\bar{X}$ with a base rate $a$. According to the Beta probability density function, the value of a FL device's opinion (trust) $i$ regarding the update $X$ during an epoch $te$ is defined as follows:  
\begin {equation}
E(O_{i \to X}^{te})=b_{i \to X}^{te}+au_{i \to X}^{te}
\end{equation}
Shard verification process can be expressed as follows: 
\begin{equation}
\
V_j(t)_=\sum_{i=1}^{n} V(t_i)E(O_{i \to t_i}^{te})
\end{equation}
where, $n$ is the number of active FL devices in a shard $j$. Every verification is weighted after being collected from a shard to the main chain for accurate reputation update. The weight of a verification is set based on multiple factors. Consequently, the traditional SL is evolved toward multi-weighted SL to consider different factors. 

To ensure a secure sharding, we expect to focus on devices with higher reputation values to train a FL model while avoiding being misled by malicious devices.
Note that the reputation of a FL device is affected by many factors among them we find interactivity and novelty. Here, we consider the following factors to calculate the trustworthiness:
\begin{itemize}
    \item Interactivity: Inside a shard, devices could either interact in a honest or dishonest manner. The honest interactions increase the trust of the device, which leads to increase the reward, and vice versa. To encourage honest behavior of FL devices, honest devices have a higher weight in the reputation process. Similarly to work \cite{r2}, the interactivity value of a device $i$ in a shard $j$ during a time epoch $te $, $S_{i}^{te}$, can be written as:
\begin{equation}
S_i^{te}=b_i^{te}+ d_i^{te}=1-u_i^{te}
\end{equation}
     \item Novelty: The trustworthiness of a FL device changes with time, the novelty is defined to measure the freshness of devices interaction inside a shard. Recent device interactions with more novelty have a higher reward than past interactions. To reflect the effect of time on reputation opinion, we define the novelty function as follows:
\begin{equation}
n_i^{te}=\nu(tn_i-te)^{-\mu}
\end{equation}
where $\nu$ and $\mu$ are two pre-defined parameters to adapt the effect of novelty, chosen similar to work in \cite{r2}. 
\end{itemize}
To sum up, by considering the interactivity and novelty, the overall weight of the reputation opinion $W_i^{te}$ of a FL device $i$ is calculated by:
\begin{equation}
f_i^{te}=w_1 n_i^{te} + w_2 S_i^{te}
\end{equation}
where $w_1$ and $w_2$ are pre-defined weight factors that satisfy $w_1 + w_2 =1$. Consequently, the reputation opinion of a FL device $i$ is aggregated with the weights factors to acquire an intra-reputation opinion denoted $w_{i,j}^{intra} = (b_{i,j}^{intra}, d_{i,j}^{intra}, u_{i,j}^{intra}, a_{i,j}^{intra})$, for a device $i$ inside shard $j$ during a time window $te\leq n$. The inter-reputation opinion is equal to the weighted reputation average of all the collected reputation opinions. The inter-reputation opinions refer to opinions that are formed after observing a targeted miner behavior. Therefore, the intra-reputation opinions of a device $i$ in a time epoch $te$ are denoted as:

\begin{equation}
\begin{cases}
b_{i,j}^{intra}= \frac{\sum_{i=1}^n f_i^{te} b_i^{te}}{\sum_{i=1}^n f_i^{te}}\\
d_{i,j}^{intra}= \frac{\sum_{i=1}^n f_i^{te} d_i^{te}}{\sum_{i=1}^n f_i^{te}}\\
u_{i,j}^{intra}= \frac{\sum_{i=1}^n f_i^{te} u_i^{te}}{\sum_{i=1}^n f_i^{te}}\\
\end{cases}
\end{equation}
and 
$E(O_{i}^{te})^{intra}=  \frac{\sum_{i=1}^n f_i^{te} E(O_i^{te}) }{\sum_{i=1}^n f_i^{te}}$ 

\subsection{Inter and Intra Reputation Process}
\begin{figure}[t]
	\centering
	\includegraphics[width=9cm, height=5cm]{figure/figure2.png}
	\caption{The operation of inter and intra reputation process.}
	\label{fig:archi}
\end{figure}
\begin{table}[t]
	
	\begin{center}
		
		\caption{SIMULATION SETUP PARAMETER}\label{tab:2}
		
		\begin{tabular}{c | c}
			\hline
			\hline
			% after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
			\textbf{Parameters} & \textbf{Value}\\
			\hline
			Classifier 
			Training examples & 1000\\
			Weight parameters  &  $\alpha$=0.4;$\beta$=0.6\\
			Epoch  & 10\\
			IP & localhost\\
			Shards &  8\\
			FL devices & 10 \\        
			PoW difficulty & 4\\
			Predefined parameters & $w_1$=$w_2$=$a$=0.5; te=60min; u=1\\
			\hline
			\hline
		\end{tabular}
		
	\end{center}
\end{table} 
The operation of the inner shard reputation aims to utilize local knowledge on the behavior of a Fl device with the other devices inside the shard. Generally, inner reputation is based on collecting reputation for centralized analysis. Consequently, we define intra-reputation and inter-reputation opinions. The intra-reputation opinion of a device $i$ is aggregated with the weight factors. As for the inter-reputation opinion is formed by other devices after observing the targeted device. To explain the basic concepts, we present a toy example of a reliable blockchain sharding for IoT systems in Fig. 2. In this example, a device $i$ has an intra-reputation opinion about an update $u$. First, the neighbor devices interact with the targeted device. Then, they form an individual opinion about it. Subsequently, they forward these opinions to the shard chain. According to the interactivity and novelty, the inter-reputation opinions are weighted. Finally, the global reputation which is equal to the joint combination of the inter-reputation and intra-reputation is updated to the main chain. If the targeted device is a new FL device inside the shard, the FL device sends a private key to the shard to be authenticated. The inter-reputation opinion $E(O_{i}^{te})^{inter}$ is calculated using other devices opinions regarding the trustworthiness of miner $i$. 


